FIRM: An Intelligent Fine-Grained Resource Management Framework for SLO-Oriented Microservices

Modern user-facing latency-sensitive web services include numerous distributed, intercommunicating microservices that promise to simplify software development and operation. However, multiplexing of compute resources across microservices is still challenging in production because contention for shared resources can cause latency spikes that violate the service-level objectives (SLOs) of user requests. This paper presents FIRM, an intelligent fine-grained resource management framework for predictable sharing of resources across microservices to drive up overall utilization. FIRM leverages online telemetry data and machine-learning methods to adaptively (a) detect/localize microservices that cause SLO violations, (b) identify low-level resources in contention, and (c) take actions to mitigate SLO violations via dynamic reprovisioning. Experiments across four microservice benchmarks demonstrate that FIRM reduces SLO violations by up to 16x while reducing the overall requested CPU limit by up to 62%. Moreover, FIRM improves performance predictability by reducing tail latencies by up to 11x.

==> prev-intro.tex <==

% the rise of containerization and microservices
Over the past decade, with the rise of containerization~\cite{senthil2017practical,merkel2014docker,container:rkt,thalheim2018cntr} and container orchestration~\cite{container:dockerswarm,container:k8s,schwarzkopf2013omega,verma2015large}, microservices have been adopted by a huge number of companies such as Netflix~\cite{microservices:netflix}, LinkedIn~\cite{microservices:linkedin}, Google~\cite{microservices:google}, and Amazon~\cite{microservices:amazon}.
Compared with monolithic designs which easily get problematic as applications get larger and more complex, microservices ease the process for software development and deployment.
Pay-as-you-go cloud computing allows each single microservice component to be scaled separately.
In addition, service owners benefit from good features brought by microservice architectures such as modularity and scalability~\cite{balalaie2015migrating,balalaie2016microservices,taibi2017processes,gan2018architectural,gan2019open}.
% single responsibility, separate of concern

% short-coming brought by microservices
However, microservices also introduce significant challenges on maintaining Service-level Objectives (SLOs) in terms of throughput or tail latency~\cite{ding2019characterizing,dean2013tail,barroso2009datacenter} which directly determine end-user experience and business revenue~\cite{sriraman2018mu,sriraman2018mutune,gan2019seer,jindal2019performance,arapakis2014impact,latencycost:money,latencycost:ranking}.
Under the pressure of SLOs, microservice owners tend to over-estimate computing resources for each container that a microservice component is deployed on~\cite{reiss2012heterogeneity}.

% bad consequences
As a result, cloud service providers such as Microsoft hit the virtual machine limit in some regions~\cite{cloudcomputinginshort}.
On the other hand, the resource utilization of modern datacenters is relatively low~\cite{reiss2012heterogeneity,barroso2009datacenter,barroso2011warehouse,delimitrou2013ibench,delimitrou2014quasar}.
It is reported that the utilization of CPU and memory in Google's datacenters are only about 35\% and 55\% respectively~\cite{reiss2011google}, implying that a large amount of the installed resources cannot be fully utilized.

% missing resource management infrastructure
Unfortunately, an ideal resource management infrastructure for microservices is missing.
Widely deployed resource managers~\cite{schwarzkopf2013omega,delimitrou2015tarcil,jyothi2016morpheus,delimitrou2013paragon,delimitrou2014quasar,qu2018auto,lorido2014review} are not targeting microservice applications.
Existing work on microservice management~\cite{container:dockerswarm,container:k8s,container:magnum,container:google,hindman2011mesos} either has trouble improving cloud resource utilization, or fails to maintain SLOs for microservices, or has its limitations.
We attribute this into two main reasons.

% why existing work sucks - reason 1
First, the scale and complexity of microservice applications make it impractical to manually determine the impact of each pair-wise dependency on end-to-end SLOs.
Instead of incorporating all functionalities into one single binary, microservices consist of hundreds or thousands of loosely-coupled service-oriented encapsulated modules~\cite{taibi2017processes,gan2019open,evolution-microservices}.
The execution paths of different types of requests are typically interleaving with each other (one component's service is needed for many other services).

% why existing work sucks - reason 2
Second, there is significant variance for cloud microservices to serve incoming requests.
Clients (request senders) perceive this as performance unpredictability.
Unpredictability has five sources: (i) resource interference, (ii) workload variation (incoming service request distribution in terms of arrival rate and request types), (iii) platform heterogeneity, (iv) network delay, and (v) software bugs.
Performance unpredictability is more noticeable and more notorious for cloud microservices~\cite{gan2019seer,gan2019open,boza2019case,yang2019miras,yu2019microscaler} because they are serving for continuous incoming client requests whose recurrent nature helps determine expected SLOs.

\begin{figure}[ht]
        \centering
        %\includegraphics[width=\linewidth]{figs/intro-slo-util.pdf}
        \includegraphics[width=\linewidth]{figs/impact.pdf}
        \caption{Performance impact of SLO violations and cluster resource utilization comparison between microservices with and without \xxx management. Microservices running in the cluster include \textit{Social Network}, \textit{Media Service}, \textit{Hotel Reservation}, and \textit{Train-ticket Booking Service}.\RED{Something wrt insight.}}
        \label{fig:eval-intro}
\end{figure}
%\begin{figure*}[ht]
    %\begin{subfigure}[b]{0.33\textwidth}
    %    \centering
    %    \includegraphics[width=\linewidth]{figs/eval-social-network.pdf}
    %    \caption[]
    %    {{\small Social Network}}    
    %    \label{fig:eval-intro-1}
    %\end{subfigure}
    %\begin{subfigure}[b]{0.33\textwidth}  
    %    \centering 
    %    \includegraphics[width=\linewidth]{example-image-a}
    %    \caption[]
    %    {{\small Media Service}}    
    %    \label{fig:eval-intro-2}
    %\end{subfigure}
    %\begin{subfigure}[b]{0.33\textwidth}   
    %    \centering 
    %    \includegraphics[width=\linewidth]{example-image-b}
    %    \caption[]
    %    {{\small Hotel Reservation}}    
    %    \label{fig:eval-intro-3}
    %\end{subfigure}
    %\begin{subfigure}[b]{0.245\textwidth}   
    %    \centering 
    %    \includegraphics[width=\linewidth]{example-image-c}
    %    \caption[]
    %    {{\small Train-Ticket Booking}}    
    %    \label{fig:eval-intro-4}
    %\end{subfigure}
    %\caption[]
    %{\small Performance impact of SLO violations and cluster resource utilization comparison between \xxx and Kubernetes auto-scaling.} 
    %\label{fig:eval-intro}
%\end{figure*}

% summary of the weakness of existing work
Cloud resource utilization requirements and performance predictability of tenant applications are poorly handled by existing systems.
Given those basic tools, microservice owners resort to a combination of ad-hoc tricks and conservatively over-provision to critical production microservices.
This lead to the tension between cloud service providers and the application owners (in this case microservices).

% auto-scalers & resource allocation
Resource allocation for single or multi-tier cloud applications essentially uses a MAPE control loop~\cite{qu2018auto,lorido2014review} to scale up and down.
When applying to microservices, it is merely impractical to break down SLOs to individual ones given the scale and complexity of the dependency graph.
Existing work on auto-scaling microservices~\cite{gias2019atom,yu2019microscaler,prachitmutita2018auto,yang2019miras} are coarse-grained and there is huge space for improving both utilization and performance predictability.
They only consider number of replicas (containers) with CPU share and memory capacity for each service.
However, containers that are co-located on the same physical machine or virtual machine have other shared resources such as Last Level Cache (LLC), network bandwidth, I\slash O, and so on.

% Tracers & RCA tools (3.3 Critical Component Extraction)
% Tracing and root-cause analysis tools help microservice owner detect and localize SLO violations, which are complementary to our work
Root-cause analysis tools~\cite{thalheim2017sieve,lin2018microscope,wu2020microrca} help microservice owner detect and localize SLO violations.
However, algorithms which are based on graph operations such as random walks, ranking, or node-wise correlation do not scale well with the microservice complexity increasing.
They have notoriously bad time complexity ($O(N^3)$, or quadratic with optimization~\cite{kang2012fast,li2012scalable}, where $N$ denotes the number of service instances).
In evaluation, it takes them nearly 4 seconds to detect and localize an anomaly, which is unacceptable in cloud microservices as the hotspots have been propagated and amplified~\cite{wu2020microrca,gan2019seer}.

Seer~\cite{gan2019seer} trains CNNs and RNNs to learn spatial and temporal patterns of SLO violations but it does not consider replica sets which are common in microservices.
In addition, prediction only 200 ms ahead of time does not make room for some actions including scale out (containers) or run micro-benchmarks to detect contentious resource.
More importantly, these approaches do not address the dynamicity in microservice environments.
Whenever a microservice changes, these approaches require burdensome model reconstruction or neural network retraining.

% proposing our work
In this paper, we move the state of art towards the ideal, by proposing a system called \xxx, which consists of a fast, lightweight inter-microservice-level SLO detection engine and a fine-grained intra-microservice-level resource adjustation backend.
Its goal is to (i) adaptively detect and localize the initiating microservice component instance of SLO violations in dynamic environments; (ii) classify the root causes into more fine-grained categories; and (iii) take actions to recover from the SLO violation.
The root cause could come from the aforementioned four sources.
We are not considering software bugs in this paper as \xxx does not require extra information about the software source code.

% === Plan A ===
% (i) find the critical path
% (ii) find the largest service on the path (which is the bottleneck, maybe the one contribute the most variance to the end-to-end latency)
% (iii) factor graph inside a container to infer the fine-grained resource limit
% (iv) for each resource, detect the optimal size

% === Plan B ===
% (i) factor graph across components to infer the culprit container
% (ii) factor graph inside a container to infer the fine-grained root cause
% (iii) optimization: mapping root cause -> action

% - software bugs (not considered)
% - platform heterogeneity (not considered)

% overview
For (i), \xxx takes a data-driven, continuously-adaptive approach to first determine critical paths leading to end-to-end SLO violations.
Based on two observed key indicators, relative importance weights and queueing congestion intensity, along with other performance-wise features, \xxx pinpoint critical service instance along each path on which container resources need to be re-adjusted.

For (ii),
%\xxx uses a novel hybrid offline and online data collection and modeling framework to provide accurate performance estimates with minimal data collection.
%Based on the estimated resources, \xxx then makes decisions on how to adjust resources without breaking SLOs and converts to cloud management actions.
\xxx utilizes a combination of offline-online data collection and modelling framework to provide accurate performance estimates and decisions with minimal data collection.
It leverages reinforcement-learning (RL) to optimize long-term reward of efficient resource allocation.% in dynamic environments.
In particular, it utilizes a model-free RL technique, i.e. a policy gradient based actor-critic approach,
to adapt to complex microservice environment dynamics.

We validate our design by implementing \xxx atop of Kubernetes~\cite{container:k8s} (\cref{eval}),
and deploy \xxx in our local cluster of 15 physical nodes.
To evaluate \xxx, we implemented four end-to-end interactive and responsive microservice benchmarks based on two open-sourced benchmark suites for cloud microservices, DeathStarBench~\cite{gan2019open} and Train-Tickets~\cite{traintickets}.
The four microservice applications are \textit{Social Network}, \textit{Media Service}, \textit{Hotel Reservation}, and \textit{Train Ticket Booking Service}.
% We intend to release components of Morpheus as open-source at "githublink".

% contribution
The paper makes the following contributions:

\begin{itemize}
\itemsep-0.3em
    \item It makes a first step towards solving the tension between application owners and cloud service providers by approaching SLO-oriented fine-grained resource management for cloud microservices.
    \item It proposes \xxx that achieves this by using data-driven analytics and model-free RL resource allocation mechanism. It describes the design (\cref{overview}) and implementation (\cref{implementation}) of \xxx. It also demonstrates its efficiency and effectiveness on maintaining SLOs and improving utilization (\cref{eval}).
    \item It presents an online critical path and component extraction (\cref{overview:critical-path}, \cref{overview:critical-component}) auto-adapting to dynamically changing microservice environments, which solves the retraining or reconstruction problem of model-based approaches.
    \item It implements a comprehensive performance fault injector (\cref{implementation:fault-injector}) that helps undercover the sources of SLO violations in cloud microservice benchmarks and helped the design of \xxx.
    \item The insights and lessons learned when designing \xxx can help microservice developer on architectural design and bottleneck analysis.
\end{itemize}

We conclude that such data-driven approaches and more fine-grained resource management are more efficient in mitigating SLO violations and improving cloud resource utilization.

% overview figure
\begin{figure}[!t]
  \includegraphics[width=\linewidth]{figs/orchestrator-overview.pdf}
  \caption{Conceptual Overview of \xxx's Architecture. Numbers matches components in \cref{overview} and \cref{implementation}}
  \label{fig:overview}
\end{figure}
